Spatio-Temporal Contrastive Self-Supervised Learning for POI-level Crowd Flow Inference

Accurate acquisition of crowd flow at Points of Interest (POIs) is pivotal for effective traffic management, public service, and urban planning. Despite this importance, due to the limitations of urban sensing techniques, the data quality from most sources is inadequate for monitoring crowd flow at each POI. This renders the inference of accurate crowd flow from low-quality data a critical and challenging task. The complexity is heightened by three key factors: 1) The scarcity and rarity of labeled data, 2) The intricate spatio-temporal dependencies among POIs, and 3) The myriad correlations between precise crowd flow and GPS reports. To address these challenges, we recast the crowd flow inference problem as a self-supervised attributed graph representation learning task and introduce a novel Contrastive Self-learning framework for Spatio-Temporal data (CSST). Our approach initiates with the construction of a spatial adjacency graph founded on the POIs and their respective distances. We then employ a contrastive learning technique to exploit large volumes of unlabeled spatio-temporal data. We adopt a swapped prediction approach to anticipate the representation of the target subgraph from similar instances. Following the pre-training phase, the model is fine-tuned with accurate crowd flow data. Our experiments, conducted on two real-world datasets, demonstrate that the CSST pre-trained on extensive noisy data consistently outperforms models trained from scratch.

==> authors-biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_ke.jpg}}]{Songyu Ke} is a PhD student in Shanghai Jiao Tong University, majoring in computer science and technology. His research interests mainly include spatio-temporal data mining with deep learning, urban computing. He is also an intern student in JD Intelligent Cities Research and JD iCity, JD Technology, Beijing, China
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_li.jpg}}]{Ting Li} received the BSc degree from the Dalian University of Technology (DUT), Dalian, Liaoning, China, in 2016, and the MSc degree from the National University of Defense Technology (NUDT), Changsha, Hunan, China, in 2019. She has worked as an algorithm engineer in JD Technology in 2019-2021. She is currently a senior algorithm engineer in AntGroup. Her current research interests include spatio-temporal data mining, time-series forecasting, automatic machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_song.jpg}}]{Li Song} is currently an algorithm engineer in JD iCity, JD Technology, Beijing, China. He received the M.S. degree from Beijing University of Posts and Telecommunications in 2019, and B.S. degree from North China Electric Power University. His research interests include spatio-temporal data mining, spatio-temporal automated machine learning and urban computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_sun.jpg}}]{Yanping Sun} is an algorithm engineer of JD Intelligent Cities Research and Intelligent Cities Business Unit, JD Digits. Her research interests mainly include urban computing, spatio-temporal data mining with deep learning and data quality improvement. She is currently mainly responsible for algorithm development and application, as well as scientific research project management. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_zhang.jpg}}]{Dr. Junbo Zhang} is a Senior Researcher of JD Intelligent Cities Research. He is leading the Urban AI Product Department of JD iCity at JD Technology, as well as AI Lab of JD Intelligent Cities Research. Prior to that, he worked at Micorsoft Research Asia from 2015 to 2018. He has published over 60 research papers in spatio-temporal data mining and AI, urban computing, deep learning, and federated learning. He serves as an Associate Editor of ACM Transactions on Intelligent Systems and Technology. He received a number of honors, including the Second Prize of the Natural Science Award of the Ministry of Education in 2021, the 22nd and 23rd China Patent Excellence Award in 2021 \& 2022, CCF Award for Science and Technology Award--Technological Progress Outstanding Award in 2021, the ACM Chengdu Doctoral Dissertation Award in 2016, the Chinese Association for Artificial Intelligence (CAAI) Excellent Doctoral Dissertation Nomination Award in 2016. He is a senior member of CCF (China Computer Federation) and IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{People/photo_zheng.jpg}}]{Yu Zheng}
is a Vice President and Chief Data Scientist at JD Technology, passionate about using big data and AI technology to tackle urban challenges. He is the general manager of the JD Urban Computing Business Unit and serves as the director of the JD Intelligent City Research. Before that, he was a senior research manager at Microsoft Research. Zheng currently serves as the Editor-in-Chief of ACM Transactions on Intelligent Systems and Technology  currently serves as the Editor-in-Chief of ACM Transactions on Intelligent Systems and Technology. He has served as chair on over 10 prestigious international conferences, e.g. as the program co-chair of CIKM 2017 (Industrial Track). In 2013, he was named one of the Top Innovators under 35 by MIT Technology Review (TR35) and featured by Time Magazine for his research on urban computing. In 2014, he was named one of the Top 40 Business Elites under 40 in China by Fortune Magazine. In 2017, Zheng was named an ACM Distinguished Scientist.
\end{IEEEbiography}
